Can Language Models Explain Their Own Classification Behavior?

Large language models (LLMs) perform well at a myriad of tasks, but explaining the processes behind this performance is a challenge. This paper investigates whether LLMs can give faithful high-level explanations of their own internal processes. To explore this, we introduce a dataset, ArticulateRules, of few-shot text-based classification tasks generated by simple rules. Each rule is associated with a simple natural-language explanation. We test whether models that have learned to classify inputs competently (both in- and out-of-distribution) are able to articulate freeform natural language explanations that match their classification behavior. Our dataset can be used for both in-context and finetuning evaluations. We evaluate a range of LLMs, demonstrating that articulation accuracy varies considerably between models, with a particularly sharp increase from GPT-3 to GPT-4. We then investigate whether we can improve GPT-3's articulation accuracy through a range of methods. GPT-3 completely fails to articulate 7/10 rules in our test, even after additional finetuning on correct explanations. We release our dataset, ArticulateRules, which can be used to test self-explanation for LLMs trained either in-context or by finetuning.

==> data/dataset-table-wide.tex <==
\begin{tabular}{@{}lccccl@{}}
\toprule
\textbf{Task} & \textbf{\# Few-shot examples} & \textbf{Size} & \textbf{Splits} & \textbf{File count} & \textbf{Details} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\textbf{Classification} &  &  &  &  &  \\
\rowcolor[HTML]{FFFFFF} 
\quad \textbf{Fine-tuning} &  &  &  &  &  \\
\rowcolor[HTML]{FFFFFF} 
\quad\quad In-distribution (\ref{app:example_prompt_in_distribution_fine_tuning}) & 32 & sm / md / lg & train / val / test & 29 & One file per rule \\
\rowcolor[HTML]{FFFFFF} 
\quad\quad Out-of-distribution (\ref{app:example_prompt_out_of_distribution_fine_tuning}) & 32 & sm / md / lg & train / val / test & 29 $\times$ 15 & One file per rule \& attack \\
\rowcolor[HTML]{EFEFEF} 
\quad \textbf{In-context} &  &  &  &  &  \\
\rowcolor[HTML]{EFEFEF} 
\quad\quad In-distribution (\ref{app:example_prompt_in_distribution_in_context}) & 32 / 64 / 128 & xs / sm / md &  & 29 & One file per rule \\
\rowcolor[HTML]{EFEFEF} 
\quad\quad Out-of-distribution (\ref{app:example_prompt_out_of_distribution_in_context}) & 32 / 64 / 128 & xs / sm / md &  & 29 $\times$ 15 & One file per rule \& attack \\
\rowcolor[HTML]{FFFFFF} 
\textbf{Articulation} &  &  &  &  &  \\
\rowcolor[HTML]{FFFFFF} 
\quad \textbf{Fine-tuning} &  &  &  &  &  \\
\rowcolor[HTML]{FFFFFF} 
\quad\quad Multiple choice (\ref{app:example_prompt_mc_articulation_fine_tuning}) & 32 & sm / md / lg & train / val / test & 29 & One file per rule \\
\rowcolor[HTML]{FFFFFF} 
\quad\quad Freeform (\ref{app:example_prompt_freeform_articulation_fine_tuning}) & 32 & sm / md / lg & train / val / test & 29 & One file per rule \\
\rowcolor[HTML]{EFEFEF} 
\quad {\color[HTML]{000000} \textbf{In-context}} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\rowcolor[HTML]{EFEFEF} 
\quad\quad {\color[HTML]{000000} Multiple choice (\ref{app:example_prompt_mc_articulation_in_context}} & {\color[HTML]{000000} 32 / 64 / 128} & {\color[HTML]{000000} xs / sm / md} & {\color[HTML]{000000} } & {\color[HTML]{000000} 29} & {\color[HTML]{000000} One file per rule} \\
\rowcolor[HTML]{EFEFEF} 
\quad\quad {\color[HTML]{000000} Freeform (\ref{app:example_prompt_freeform_articulation_in_context})} & {\color[HTML]{000000} 32 / 64 / 128} & {\color[HTML]{000000} xs / sm / md} & {\color[HTML]{000000} } & {\color[HTML]{000000} 29} & {\color[HTML]{000000} One file per rule} \\ \bottomrule
\end{tabular}

